Tests of Scintillator+WLS strips for Muon System at Future Colliders

Prototype scintilator+WLS strips with SiPM readout for muon system at future colliders were tested for light yield, time resolution and position resolution. Depending on the configuration, light yield of up to 36 photoelectrons per muon per SiPM has been achieved, as well as time resolution of 0.5 ns and position resolution of ~7 cm.

==> include/Speed_1.tex <==
\subsubsection{Speed of light along the strip}
\label{sec:speed1}



==> include/Speed_2.tex <==
\subsubsection{Speed of light along the strip}
\label{sec:speed2}


